CrowdSpeech and VoxDIY: Benchmark Datasets for Crowdsourced Audio Transcription

Domain-specific data is the crux of the successful transfer of machine learning systems from benchmarks to real life. In simple problems such as image classification, crowdsourcing has become one of the standard tools for cheap and time-efficient data collection: thanks in large part to advances in research on aggregation methods. However, the applicability of crowdsourcing to more complex tasks (e.g., speech recognition) remains limited due to the lack of principled aggregation methods for these modalities. The main obstacle towards designing aggregation methods for more advanced applications is the absence of training data, and in this work, we focus on bridging this gap in speech recognition. For this, we collect and release CrowdSpeech -- the first publicly available large-scale dataset of crowdsourced audio transcriptions. Evaluation of existing and novel aggregation methods on our data shows room for improvement, suggesting that our work may entail the design of better algorithms. At a higher level, we also contribute to the more general challenge of developing the methodology for reliable data collection via crowdsourcing. In that, we design a principled pipeline for constructing datasets of crowdsourced audio transcriptions in any novel domain. We show its applicability on an under-resourced language by constructing VoxDIY -- a counterpart of CrowdSpeech for the Russian language. We also release the code that allows a full replication of our data collection pipeline and share various insights on best practices of data collection via crowdsourcing.

==> rant.tex <==
Our current approach:

\begin{itemize}
    \item Take WikiText and BookCorpus
    \item Filter out poor-formatted sentenses, sentences with weird names etc.
    \item Record texts using Yandex Speech Kit
    \item Annotate recordings on Toloka
\end{itemize}

Some critical questions:

Q1: \emph{Why do we use some strange pool of texts instead of annotating LibriSpeech -- a well known benchmark for speech recognition.}

A1: We did not want to use LibriSpeech because of the contest (test labels would be compromised). \textbf{Note that this answer is not valid for NeurIPS submission --- we must provide excellent quality data and the contest is not a good reason to decrease the quality of data. Our current data does not fit exactly (see Q2 below).}

A2: In practice, people may need more data than in LibriSpeech to train super large networks. Additionally, people may want to consturct different datasets to test their models in a different domain. Thus, (i) we provide an end-to-end pipeline to obtain recordings as well as annotations of these recordings without having real people recording audios. \textbf{This makes sense if written carefully, BUT largely as an additional thing to LibriSpeech. To make this point, we need to annotate LibriSpeech as well.}

\bigskip

Q2: \emph{Why your filtering procedure is so vague -- you tried to filter something but did not manage to do it completely?}

A: Right, for the sake of the contest, we did some light filtering and did not want to make it 100\% complete. \textbf{Note that this explanation does not work for a paper. If we want to filter something, we need to have a good reason and need to filter things properly.}

Q3: \emph{Does using Speech Kit result in a semi-realistic data? What if ppl do make different mistakes when annotating real audios?}

A: Good point, we dont know. But we can annotate LibriSpeech to show that methods that perform well on our data are also good on LibriSpeech. \commentivan{Need to do this!}


\commentivan{All in all, it seems that because we wanted to support the contest, we made some choices that are suboptimal for the paper (e.g., poorly-formulated filtering, decision to not label benchmarks). Additionally, we did not polish the pipeline and instructions of our tasks --- they are not exemplary!!!.}


\commentivan{One work around would be to (i) annotate librispeech benchmark, (ii) polish our filtering procedure and provide end-to-end pipeline for a user to obtain additional annotations of WikiText and BookCorpus.}

\commentivan{Additionally, in August we will be able to say that we've hosted a competition and, HOPEFULLY, say that in this competition there are methods that already provide improvements over the baseline. This would be a very strong point so I think we should wait till the end of the competition}

\commentivan{Finally, by releasing the paper we will release the source of the contest data which is kind of a data leak that is not super cool for the sake of the contest.}

\commentivan{Overall, Given that there is a sufficient amount of work to properly fix the issues outlined above + we need to do a bunch of work on preparing code for end-to-end annotation, i am inclined to postpone the submission till the second ddl in august}

